Pareto optimal and popular house allocation with lower and upper quotas

In the house allocation problem with lower and upper quotas, we are given a set of applicants and a set of projects. Each applicant has a strictly ordered preference list over the projects, while the projects are equipped with a lower and an upper quota. A feasible matching assigns the applicants to the projects in such a way that a project is either matched to no applicant or to a number of applicants between its lower and upper quota. In this model we study two classic optimality concepts: Pareto optimality and popularity. We show that finding a popular matching is hard even if the maximum lower quota is 2 and that finding a perfect Pareto optimal matching, verifying Pareto optimality, and verifying popularity are all NP-complete even if the maximum lower quota is 3. We complement the last three negative results by showing that the problems become polynomial-time solvable when the maximum lower quota is 2, thereby answering two open questions of Cechl\'arov\'a and Fleiner. Finally, we also study the parameterized complexity of all four mentioned problems.

==> inclusions.tex <==
\usepackage{color}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{amsmath}
\usepackage{amsthm}
\interdisplaylinepenalty=2500
\usepackage{amssymb,amsfonts,textcomp}
\usepackage{latexsym}
\usepackage{graphicx} 
\usepackage{multirow}
\usepackage{microtype}
\usepackage{float}
\usepackage{rotating}
\usepackage{url}
\usepackage{color}
\usepackage{comment}
\usepackage{paralist}
\usepackage{booktabs}
\usepackage{bm}
\usepackage[]{units}
\usepackage[noend, ruled, noline]{algorithm2e}
\usepackage{tikz}
\usepackage[sort&compress,comma,numbers]{natbib}
\usepackage{lmodern}
\usepackage{mathtools}
\usepackage{cleveref}
\usepackage{rotating,tcolorbox,complexity}
\usepackage{thmtools}
\usepackage{thm-restate}
\declaretheorem[name=Theorem,numberwithin=section]{thm}
\declaretheorem[name=Corollary,numberwithin=section]{cor}
\declaretheorem[name=Observation,numberwithin=section]{obs}
\declaretheorem[name=Lemma,numberwithin=section]{lem}



\usepackage{boxedminipage}
\usepackage{xspace}
\newcommand{\pbDef}[3]{%
			\noindent
			\begin{center}
			\begin{tcolorbox}
			\vspace{-2mm}
			#1\\%[5pt]
			\begin{tabular}{p{0.1\columnwidth}p{0.8\columnwidth}}
			Input: & #2\\
			Question: & #3
			\end{tabular}\vspace{-2mm}
			\end{tcolorbox}
			\end{center}
			}
\newcommand{\optPDef}[3]{%
			\noindent
			\begin{center}
			\begin{tcolorbox}
			\vspace{-2mm}
			#1\\%[5pt]
			\begin{tabular}{p{0.1\columnwidth}p{0.8\columnwidth}}
			Input: & #2\\
			Task: & #3
			\end{tabular}\vspace{-2mm}
			\end{tcolorbox}
			\end{center}
			}


\sloppy
\allowdisplaybreaks

\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\Ie}{I.e.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\problemdef}[4]{
	\begin{center}
		\begin{minipage}{0.95\textwidth}
			\normalsize\textsc{#2} \smallskip \\
			\begin{tabularx}{\textwidth}{@{}l@{\hspace{3pt}}X}
				\normalsize\textbf{Input:} & \normalsize#3 \\
				\normalsize\textbf{#1:}    & \normalsize#4
			\end{tabularx}
		\end{minipage}
	\end{center}
}
\newcommand{\dprob}[4][Question]{\problemdef{#1}{#2}{#3}{#4}}
\newcommand{\optprob}[4][Task]{\problemdef{#1}{#2}{#3}{#4}}
\DeclareMathOperator{\vote}{vote}

\newenvironment{proofsketch}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}



\newcommand{\integers}{{{\mathbb{Z}}}}
\newcommand{\naturals}{{{\mathbb{N}}}}
\newcommand{\rationals}{{{\mathbb{Q}}}}
\newcommand{\wone}{{\mathrm{W[1]}}}
\newcommand{\w}{{\mathrm{W}}}
\newcommand{\fpt}{{\mathrm{FPT}}}
\newcommand{\np}{{\mathrm{NP}}}
\newcommand{\paranp}{{\mathrm{paraNP}}}
\newcommand{\conp}{{\mathrm{coNP}}}
\newcommand{\av}{{\mathrm{av}}}
\newcommand{\vecw}{{\mathbf{w}}}
\newcommand{\lin}{\cal{L}}
\newcommand{\calh}{\mathcal{H}}
\newcommand{\ct}{\textsc{c3dsm} \xspace}
\newcommand{\Mp}{M^\prime}
\newcommand{\hopen}{P_{\text{open}}}
\newcommand{\mquota}{m_{\text{quota}}}
\newcommand{\mopen}{m_{\text{open}}}
\newcommand{\hquota}{P_{\text{quota}}}
\newcommand{\mclosed}{m_{\text{closed}}}
\newcommand{\lmax}{\ell_{\text{max}}}
\newcommand{\umax}{u_{\text{max}}}
\newcommand{\degA}{\Delta_A}
\newcommand{\degH}{\Delta_P}
\newtheorem{oquestion}{Open Question}
\newcounter{captionedequationset} %
\newdimen\captionlength
\newcommand{\captionedequationset}[1]{
    \refstepcounter{captionedequationset}%
    \setlength{\captionlength}{\widthof{#1}} %
    \addtolength{\captionlength}{\widthof{Equation set~\thecaptionedequationset: }}
    \ifthenelse{\lengthtest{\captionlength < \linewidth }} %
    {\begin{center}
            Preference structure~\thecaptionedequationset: #1
        \end{center}} 
    { \begin{flushleft} 
        Preference structure~\thecaptionedequationset: #1 %
        \end{flushleft}}}
\newcommand{\popular}{\textsc{pop-ha$_L^U$\;}}
\newcommand{\popver}{\textsc{popv-ha$_L^U$\;}}
\newcommand{\maxpareto}{\textsc{perpo-ha$_L^U$\;}}
\newcommand{\parver}{\textsc{pov-ha$_L^U$\;}}
\newcommand{\wmatch}{\textsc{w-ha$_L^U$\;}}

\newcommand{\popularnsp}{\textsc{pop-ha$_L^U$}}
\newcommand{\popvernsp}{\textsc{popv-ha$_L^U$}}
\newcommand{\maxparetonsp}{\textsc{perpo-ha$_L^U$}}
\newcommand{\parvernsp}{\textsc{pov-ha$_L^U$}}
\newcommand{\wmatchnsp}{\textsc{w-ha$_L^U$}}
\usepackage[textsize=tiny,textwidth=2cm,shadow]{todonotes}
\newcommand{\accom}[1]{\todo[color=green!20!white]{\'{A}: #1}}
\newcommand{\jpcom}[1]{\todo[color=yellow!40!white]{{J}: #1}}
\newcommand{\tfcom}[1]{\todo[color=blue!20!white]{{T}: #1}}
